Scaling Ordered Stream Processing on Shared-Memory Multicores

Many modern applications require real-time processing of large volumes of high-speed data. Such data processing needs can be modeled as a streaming computation. A streaming computation is specified as a dataflow graph that exposes multiple opportunities for parallelizing its execution, in the form of data, pipeline and task parallelism. On the other hand, many important applications require that processing of the stream be ordered, where inputs are processed in the same order as they arrive. There is a fundamental conflict between ordered processing and parallelizing the streaming computation. This paper focuses on the problem of effectively parallelizing ordered streaming computations on a shared-memory multicore machine. We first address the key challenges in exploiting data parallelism in the ordered setting. We present a low-latency, non-blocking concurrent data structure to order outputs produced by concurrent workers on an operator. We also propose a new approach to parallelizing partitioned stateful operators that can handle load imbalance across partitions effectively and mostly avoid delays due to ordering. We illustrate the trade-offs and effectiveness of our concurrent data-structures on micro-benchmarks and streaming queries from the TPCx-BB benchmark. We then present an adaptive runtime that dynamically maps the exposed parallelism in the computation to that of the machine. We propose several intuitive scheduling heuristics and compare them empirically on the TPCx-BB queries. We find that for streaming computations, heuristics that exploit as much pipeline parallelism as possible perform better than those that seek to exploit data parallelism.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

==> sections/FutureWork.tex <==
\section{Conclusions and Future Work}
\label{sec:future-work}
There are several interesting extensions to our work but we focus on two of them here. 
One very important extension is to design scheduling heuristics that discriminate workers based on their spatial locality. In our current scheme, we essentially assume all worker threads are uniform. However, in reality a worker is closer to some workers than others due to the hierarchical cache architecture. This distinction between workers becomes very important when we have non-uniform memory access (NUMA). In some of our experiments, we observed that the overhead of parallelizing a data parallel operator on cores across NUMA nodes shoots up dramatically. 
\par 
Another direction for future work is handling more complicated DAGs than just linear chains. In most cases, it is straight-forward to generalize our priority-based heuristics to a DAG. However, in some cases, the operator semantics complicate the flow and hence may lead to unnecessary stagnation. For example, consider a \texttt{pairwise-join} operator: it needs one input from each of its edges to compute an output, which means the scheduling heuristic needs to schedule operators that produce inputs along all its edges in tandem. Such requirements might not be addressed using the simple heuristics we discussed earlier. 

==> sections/Ordering.tex <==
\section{Ordering and Parallelization}
\label{sec:ordering}
 The scheduler in our runtime may allot more than one worker to the same operator at a time, which necessitates concurrent processing of inputs from the worklist of an operator.
 This applies only to stateless and partitioned stateful operators, as the maximum allowed degree of parallelism for a stateful operator is 1. 
 In order to support concurrent workers efficiently, we need to design a scalable, low-overhead parallelization scheme for such operators. 
Our focus is on \emph{ordered} stream processing, which further adds interesting challenges in designing this framework.
 We discuss these issues and present some concurrent data structures that help achieve this. 
 \par
Stateful operators are processed by at most a single worker hence, ensuring ordered processing is straight-forward. 
In case of stateless and partitioned stateful operators, however, multiple workers process inputs concurrently and so they need special constructs to ensure this constraint. 
There are essentially two kinds of ordering requirements that must be handled correctly. 
The first kind is \emph{processing order}: for some operators we need to ensure that the tuples are processed in the same order as they arrive. 
This is a key requirement for non-commutative stateful operators. 
On the other hand, there is no such constraint for stateless operators. 
Partitioned stateful operators present an interesting middle-ground where it is enough to guarantee that tuples with the same key are processed in their arrival order. 
\par 
The second kind of requirement is \emph{output ordering}, which specifies that the outputs of an operator are sent to the downstream operator in the same order as its inputs. 
We need to ensure this property for both stateless and partitioned stateful operators. 
In particular, even when input tuples $i_1$ and $i_2$ can be processed concurrently (when they belong to different partitions or when the operator is stateless): we still need to ensure that the outputs $o_1$ and $o_2$ produced by these inputs are sent out in the right order. 
We describe a low-overhead, non-blocking solution to this problem in section \ref{sec:reordering-scheme}.
\par
Output ordering is innately a blocking constraint: even if $o_2$ is produced before $o_1$, it gets blocked until $o_1$ is produced and sent downstream.  
 This manifests as an implicit advantage for parallelization schemes that processes inputs from the worklist \emph{almost} in the order of their arrival even though the semantics does not impose a restriction on this order. For stateless operators, having a shared worklist directly enables this execution pattern. However, it is non-trivial to achieve this for partitioned stateful operators. We present an adaptive partitioning scheme that supports this notion of almost ordered processing in the next section.
